Correction and standardisation of lung oscillometry techniques using parameter inference: A study group report

This report relates to a study group hosted by the EPSRC funded network, Integrating data-driven BIOphysical models into REspiratory MEdicine (BIOREME), and supported by The Insigneo Institute and The Knowledge Transfer Network. The BIOREME network hosts events, including this study group, to bring together multi-disciplinary researchers, clinicians, companies and charities to catalyse research in the applications of mathematical modelling for respiratory medicine. The goal of this study group was to provide an interface between companies, clinicians, and mathematicians to develop mathematical tools to the problems presented. The study group was held at The University of Sheffield on the 17 - 20 April 2023 and was attended by 24 researchers from 13 different institutions. This report relates to a challenge presented by Arete Medical Technologies relating to impulse oscillometry (IOS), whereby a short pressure oscillation is imposed at a person's mouth during normal breathing, usually by a loudspeaker. The resulting pressure and flow rate changes can be used to the impedance of the airways, which in turn can provide proxy measurements for (patho)physiological changes in the small airways. Disentangling the signal so that airway mechanics can be measured accurately (and device properties/environmental effects can be accounted for) remains an open challenge that has the potential to significantly improve the device and its translation to clinic. In this report, several approaches to this problem, and the wider problem of interpreting oscillometry resuts are explored.

==> sources/9_nomenclat.tex <==
\makenomenclature
%\clearpage
%\mbox{}

% \nomenclature{EV}{Electric Vehicle}
% \nomenclature{AC}{Alternating Current}
% \nomenclature{DC}{Direct Current}
% \nomenclature{IGBT}{Insulated-gate Bipolar Transistor}
% \nomenclature{PV}{Photovoltaics}
% \nomenclature{RMS}{Root Mean Square}
% \nomenclature{FCS}{Fast Charging Station}
% \nomenclature{PMU}{Phase Measurement Unit}
% \nomenclature{THD}{Total Harmonic Distortion}
% \nomenclature{EMI}{Electromagnetic Interference}
% \nomenclature{$h$}{Planck constant}
 
\printnomenclature
